Dynamic Model Predictive Shielding for Provably Safe Reinforcement Learning

Among approaches for provably safe reinforcement learning, Model Predictive Shielding (MPS) has proven effective at complex tasks in continuous, high-dimensional state spaces, by leveraging a backup policy to ensure safety when the learned policy attempts to take risky actions. However, while MPS can ensure safety both during and after training, it often hinders task progress due to the conservative and task-oblivious nature of backup policies. This paper introduces Dynamic Model Predictive Shielding (DMPS), which optimizes reinforcement learning objectives while maintaining provable safety. DMPS employs a local planner to dynamically select safe recovery actions that maximize both short-term progress as well as long-term rewards. Crucially, the planner and the neural policy play a synergistic role in DMPS. When planning recovery actions for ensuring safety, the planner utilizes the neural policy to estimate long-term rewards, allowing it to observe beyond its short-term planning horizon. Conversely, the neural policy under training learns from the recovery plans proposed by the planner, converging to policies that are both high-performing and safe in practice. This approach guarantees safety during and after training, with bounded recovery regret that decreases exponentially with planning horizon depth. Experimental results demonstrate that DMPS converges to policies that rarely require shield interventions after training and achieve higher rewards compared to several state-of-the-art baselines.

==> algo.tex <==
\begin{algorithm}[t]
\footnotesize
\caption{TD3 with Dynamic Recovery Planning}
\label{algo:training}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} 
%($\mathcal{M}$: Markov Decision Process), 
(Episode Count: $E$)
%, ($\pi_r$: Task-oblivious Recovery Policy)

\STATE  $\pi_\theta, Q_{\phi_1}, Q_{\phi_2} := \mathtt{initNetworks()}$ \algcmt{Initialize one actor and two critic networks.}
\STATE $\theta^{t}, \phi_1^{t}, \phi_{2}^{t} := \mathtt{initTargets}()$ \algcmt{Initialize target networks for soft updates.}
\STATE $\mathcal{B} := \emptyset$ \algcmt{Initialize an empty replay buffer.}

\FOR{$e \in [1,E]$}

    \STATE $s := \mathtt{beginEpisode}(e)$ \algcmt{Initialize a new episode and get the first observed state.}
    \WHILE{$\neg \mathtt{terminated}(e)$} 
        \STATE  $a_{\text{next}} := \pi_{\theta}(s) + \mathcal{N}(0, \sigma)$ \algcmt{Choose a candidate action using the base policy with normal noise.}
        \IF{$\mathcal{T}(s,a_{\text{next}})\not\in\mathcal{S}_{{rec}}^{\pi_r}$ }
        \STATE $\mathcal{B} := \mathcal{B}\cup \langle s, a_{\text{next}}, \varnothing, r^-\rangle$ \algcmt{Add a record with a large negative penalty to the buffer.}
       \STATE \textbf{if}  $a_{1:n} = \mathtt{planRec}(s,Q_{\phi_1}) $ \textbf{then} $a_{\text{next}} := a_1$ \algcmt{Plan recovery and choose the next action.}
        \STATE \textbf{else}  $a_{\text{next}} := \pi_r(s)$ \algcmt{Use the task-agnostic recovery policy if planning fails.}
        \ENDIF
        \STATE $s', r := \mathtt{execute}(s,a_{\text{next}})$ \algcmt{Execute the selected next action on the environment.}
        \STATE $\mathcal{B} := \mathcal{B}\cup \langle s, a_{\text{next}}, s', r\rangle$ 
        \algcmt{Update the buffer with the recent transition record.}
        \STATE $s := s'$

    \ENDWHILE
    \STATE $\mathtt{updateNetworks}(\pi_\theta, Q_{\phi_1}, Q_{\phi_2}, \mathcal{B}) $  \algcmt{Update networks using gradient descent.}
    \STATE $\mathtt{updateTargets}(\theta^{t}, \phi_1^{t}, \phi_{2}^{t})$ \algcmt{Update target parameters using Polyak averaging.}
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> benchmark_description_table.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Safety Results}
\label{tab:behcn_desc}
\begin{tabular}{@{}|p{7mm}l|ccccc|cc|}
\hline
 \multicolumn{2}{|c|}{\multirow{2}{*}{\bf Benchmark}} & \multicolumn{5}{c|}{\textbf{\# Shield Invocations / Episode}} & \multicolumn{2}{c|}{\textbf{\# Safety Violations}} \\
&           & DMPS & DMPS-H1 & MPS & MPS-G & REVEL & CPO & TD3 \\ \hline
\multirow{6}{*}{\rotatebox{0}{Static}} & \texttt{obstacle}           & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{obstacle2}          & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{mount-car}       & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{pendulum}           & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{road}               & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{road2d}             & a    & b       & c   & d     & e     & f   & g   \\\hline
   \multirow{4}{*}{\rotatebox{0}{\parbox{1cm}{Double \\ Integrator}}}                      & \texttt{dynamic-obs}   & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{single-gate}               & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{double-gates}        & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{double-gates+}  & a    & b       & c   & d     & e     & f   & g   \\\hline
\multirow{4}{*}{\rotatebox{0}{Steering}}                        & \texttt{dynamic-obst}   & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{single-gate}        & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{double-gates}  & a    & b       & c   & d     & e     & f   & g   \\
                         & \texttt{double-gates+}   & a    & b       & c   & d     & e     & f   & g   \\
\hline
\end{tabular}
\end{table}

==> double_gates_plus_plots.tex <==
\setlength{\figheight}{29mm} % Adjust the value as needed
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_Steering.png}}
        \caption*{Shield Invocations (DD)}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_Steering.png}}
        \caption*{Performance (DD)}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_DoubleIntegrator.png}}
        \caption*{Shield Invocations (DI)}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_DoubleIntegrator.png}}
        \caption*{Performance (DI)}
        \label{}
    \end{subfigure}
    \caption{Performance and shield invocation trajectories in \texttt{double-gate+} environment.}
    \label{fig:double_gate_plus_plots}
\end{figure}


==> double_gates_plus_plots_separate.tex <==
\setlength{\figheight}{29mm} % Adjust the value as needed

\begin{figure}[b]
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_Steering.png}}
            \caption{Differential Drive}
            \label{fig:sub1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_DoubleIntegrator.png}}
            \caption{Double Integrator}
            \label{fig:sub2}
        \end{subfigure}
        \caption{Shield Invocations in \texttt{double-gate+}}
        \label{fig:shield_plots}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_Steering.png}}
            \caption{Differential Drive}
            \label{fig:sub3}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_DoubleIntegrator.png}}
            \caption{Double Integrator}
            \label{fig:sub4}
        \end{subfigure}
        \caption{Performance in \texttt{double-gate+}}
        \label{fig:perf_plots}
    \end{minipage}
\end{figure}





==> files/arkos_theorems.tex <==
%%%% HERE ARE ARKO'S STUFF RELATING THEOREMS
\begin{comment}
We assume that the $\textsc{Plan}(s_t)$ protocol bounded to $n$ step trajectories returns a path $(a_t, a_{t+1}, \dots, a_{t+n-1})$ maximizing the $n-1$-step return from the input state. Here, the $n-1$-step return is $G_{t:t+n-1} = R_{t+1} + \gamma \cdot R_{t+2} + \gamma^2 \cdot R_{t+3} + \dots + \gamma^{n-2} \cdot R_{t+n-1} + \gamma^{n-1} \cdot Q(s_{t+n-1}, a_{t+n-1}).$

\begin{theorem}
\label{th:op}
Fix some state $s_t \in \mathcal S$ and let $(a_t, \dots, a_{t+n})$ be the output of $\textsc{Plan}(s_t)$ bounded to $n-1$-step trajectories. Let $G^\star$ be the optimal infinite horizon return from $s_t$ and $G'$ be the optimal infinite horizon from $s_t$ on the condition that the path must begin with the actions $(a_t, \dots, a_{t+n}).$ Let $Q^\star$ be the optimal $Q$ function. Then:

\begin{enumerate}
	\item Under the assumption that $Q$ is $\epsilon$-close to $Q^\star,$ we have $|G' - G^\star| = O(\epsilon \gamma^n).$
    \item Under the assumption that $\mathcal S$ is compact and both $Q$ and $Q^\star$ are continuous, we have $|G' - G^\star| = O(\gamma^n).$
    \item Under the assumption that the maximum reward at any timestep is bounded, we have $|G' - G^\star| = O(\gamma^n).$
    \item Under the assumption that $\|\mathcal T(s,a) - s\|$ is bounded (a reasonable assumption for Physics-based environments), and that $Q$ and $Q^\star$ are Lipschitz continuous, we have $|G' - G^\star| = O(n \gamma^n).$
\end{enumerate}
\end{theorem}



One can think of the proposed algorithm as solving a modified MDP $\mathcal M'$ that is derived from $\mathcal M,$ except that $\mathcal R_{\mathcal M'}(s,a,s') = \begin{cases} R_{\mathcal M}(s,a,s') & s' \in \mathcal S_{rec} \\ R^-  & \text{otherwise} \end{cases}.$

\begin{theorem}
\red{this is more like a lemma}
Let $R$ be the minimum reward that can be assigned to a timestep under the MDP $\mathcal M.$ Suppose that $R^- < \frac{R}{1-\gamma}.$ Finally, suppose that the algorithm converges to a policy $\pi^\star$ that solves $\mathcal M'$ optimally. Then $\pi^\star$ never faces shield triggers.
\end{theorem}

\begin{theorem}
\label{th:regret}
    Let $R$ be the minimum reward that can be assigned to a timestep under the MDP $\mathcal M.$ Suppose that $R^- < R.$ [INSERT CONTINUITY ASSUMPTIONS]

Suppose the algorithm converges to a policy $\pi_\theta$ that is a locally optimal solution to $\mathcal M'.$ Further, define $S(\theta)$ to be the expected number of shield triggers invoked by the policy $\pi_\theta.$ Then, $\theta$ is a local minimum of $S.$
\end{theorem}
\end{comment}












%%%% BELOW IS THE OLD ALGORITHM (ARKO'S INITIAL VERSION)
\begin{comment}

\begin{algorithm}[t]
\scriptsize
\caption{\red{OLD MCTS (to be removed)}}
\begin{algorithmic}[1]

\STATE \textbf{Inputs:} ($s_0$: start state), ($Q$: state-action function), ($K$: number of samples), ($M$: number of expansions \red{maybe number of iterations}), ($L$: maximum path length \red{another way to constrain exploration})

\STATE Initialize hashmaps $\hat Q : \mathcal S \times \mathcal A \to \mathbb R \red{\text{ estimate of the Q function within the algo which is updated at each iteration}}, N : \mathcal S \times \mathcal A \to \mathbb N.\red{\text{something that is used for balancing exploration and exploitation}}$
\STATE Initialize MCTS tree $T$ with  vertex $s_0$ \red{\text{nodex are states edges are actions}}
\STATE $\texttt{expand}(s_0, \hat{Q}, Q,  K , T)$ \red{\text{perform an expansion starting from $s_0$ and update the Tree and estimate of Q and N}}
\FOR {$t \gets 1 \text{ to } M$}
    \STATE Select $s_0, a_0, R_0, s_1, a_1, R_1, \dots, s_r = NIL$ \red{\text{means that $s_r$ is not yet on the tree but $s_{r-1}$ is a leaf node }} using $\hat Q+UCT$ selection. \red{\text{this line simply chooses a path from root to a leaf based on explo-exploit balance}}
    \IF {$r < L$} 
        \STATE Set $s_r \gets \mathcal T(s_{r-1}, a_{r-1})$ in $T$. \red{\text{if we update T so ends with actual states then this line is not necessary}}
        \STATE $\texttt{expand}(s_r)$ \red{\text{remember: $\hat{Q}$ value is updated here}}
        \STATE $a_r$ := Select from outgoing actions from $s_r$ via $\hat Q+UCT$ selection.
    \ENDIF
    \STATE Set horizon $H$ to $r$ if $r < L$ and $r-1$ otherwise.
    \STATE For $1 \leq i \leq r - 1,$ update $\hat Q(s_i, a_i) \gets \frac{1}{N(s_i,a_i)+1}\left[N(s_i, a_i)\hat Q(s_i,a_i) + \left((\sum_{j=i}^{H-1} \gamma^{j-i} \cdot R_j) + \gamma^{H-i} \hat Q(s_H, a_H)\right)\right]$
    \STATE For $1 \leq i \leq r - 1,$ update $N(s_i,a_i) \gets N(s_i,a_i) + 1$
\ENDFOR

\STATE Select $s_0, a_0, s_1, a_1, \dots, s_m, a_m$ greedily using $\hat Q$ selection

\STATE Return $(a_0, \dots, a_m)$

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\scriptsize
\caption{EXPAND}
\begin{algorithmic}[1]

\STATE \textbf{Inputs:} ($s$: state), ($Q$: state-action function), ($K$: number of samples), ($T$: MCTS tree)

\STATE Sample $a_1, \dots, a_K \sim \mathcal A$ \red{\text{here we actually filter out non-recoverable }}
\STATE Set $\hat Q(s_0, a_i) \gets Q(s_0, a_i)$ for $1 \leq i \leq K$
\STATE Set $N(s_0, a_i) = 1$ for $1 \leq i \leq K.$
\STATE For $1 \leq i \leq K,$ add an edge in $T$ from $s_0$ to a NIL vertex using action $a_i.$

\end{algorithmic}
\end{algorithm}


\end{comment}

==> files/deprecated.tex <==
%unlike $\pi_\text{mps}$, which would resort to using the recovery policy (as shown in \autoref{subfig:example_brake}), the policy $\pi_\tool$ first attempts to plan for more optimal recovery actions.
%
%\red{todo: elaborate the example. The example should show the intrinsic behavior of MCTS and clearly show why a planner -- as opposed to a greedy selection -- is needed}. 


%if the planner cannot identify any recoverable action within the given resource limits.


%In theory any planning algorithm can be used here, 

%an \textit{dynamic recovery planner} that aims to identify a sequence of actions which maximize the  discounted expected recovery value with respect to the given Q function. 

%\red{[todo: Elaborate sampling, failure possibility, objectives. Mention MCTS but say that others would work too.]}
%
%Specifically, the choice of recovery action in $\pi_r^*$ is informed by $\bar{Q}:\mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$, which is the so-called \textit{safety-neutral} action-value function (\ie{} the Q-function) of the given task. 
%This safety-neutral Q-function represents the expected infinite-horizon discounted reward of executing an action in a particular state, over an MDP that preserves the reward structure of $\mathcal{M}$, but relaxes its safety constraints. 
%
%\red{todo: cite and discuss \cite{zhang2020cautious}}






%More formally, the informed recovery policy $\pi^*_{r}$ performs a sampling-based search for an action with maximum value with respect to $\bar{Q}$, \ie{} 
%$$
%\pi_r^*(\bar{Q},s) \doteq \argmax_{a \in \mathtt{sampleRecAct}(s) \cup \{\pi_r(s)\}} \bar{Q}(s,a)
%$$
%In the above definition, $\mathtt{sampleRecAct}$ returns a set of $n$ actions that are recoverable from $s$, \ie{} 
%$\mathtt{sampleRecAct}(s) \doteq \{a_1, \dots, a_n\} \subseteq \mathcal{A}$,
%such that $\forall_{1\leq i\leq n}.\; \mathcal{T}(s,a_i) \in \mathcal{S}_{{rec}}$, and $n$ is a hyper-parameter. 
%






%\todo{this discussion seems out of place}
%
%Thus our approach guarantees safety similar to $\pi_\text{mps}$, however, 
% it is capable of finding more optimal recovery paths than $\pi_\text{mps}$.
 % compared to$\pi_r$.

%For example, three sampled actions from this state and their corresponding progress values with respect to $\bar{Q}$ are shown. The action $a_2$ (shown in red) does not lead to a recoverable state and is thus excluded from consideration.  From the remaining actions, $a_3$ (shown in green) is selected as the optimal recovery action, since it leads to a recoverable state and has a higher progress value than $a_1$. By repeating this process in the subsequent states, the policy $\pi_\text{imps}$ is  able to effectively navigate around the obstacle towards the goal, similar to the trajectory depicted in \autoref{fig:example}~(c).

%Following is a theorem stating the safety and the asymptotic optimality of our approach with respect to $\bar{Q}$. The proof is straightforward and is given in  \autoref{app:proof}.

==> files/performance_table_rebuttal.tex <==
\newlength{\colwidthperfXYZ}
\setlength{\colwidthperfXYZ}{1mm} % You can adjust the value as needed
   % \centering
\begin{table}[h]
    \centering
    \scriptsize
    \caption*{Table 2: Updated Performance Results}
    \label{tab:perf}
    \begin{tabular}{|cl|rr|rr|rr|rr|rr|rr|}
        \hline
        \multicolumn{2}{|c|}{\multirow{3}{*}{\bf Bdenchmark}} & 
        \multicolumn{12}{c|}{\textbf{Total Return in Final 10 Episode}}\\ \cline{3-14} 
        &           & 
        \multicolumn{2}{|c|}{\tool} & 
       % \multicolumn{2}{|c|}{\texttt{DMPS-H1}}  & 
        \multicolumn{2}{|c|}{\texttt{MPS}} & 
       % \multicolumn{2}{|c|}{\texttt{DMPS-G}}  & 
        \multicolumn{2}{|c|}{\texttt{REVEL}}  & 
        \multicolumn{2}{|c|}{\texttt{CPO}}  & 
        \multicolumn{2}{|c|}{\texttt{PPO-Lag}}  & 
        \multicolumn{2}{|c|}{\texttt{TD3}} \\
        &           & 
        mean & sd & 
        mean & sd &  
       % mean & sd & 
        mean & sd &  
        mean & sd &  
        mean & sd &  
        mean & sd \\
        \hline
        \multirow{5}{*}{\rotatebox{0}{ST}} 
        & \texttt{obstacle} & 
        $32.7$ & $0.3$ & 
        %$31.9$ & $1.0$ & 
        $8.6$ & $47.9$ & 
        %$32.43$ & $0.73$ & 
        $-41.6$ & $52.7$ & 
        $32.8$ & $0.0$ &
        $32.8$ & $0.4$ &
        $\mathbf{32.9}$ & $0.0$ \\
        & \texttt{obstacle2} & 
        $20.2$ & $15.2$ & 
        %$6.81$ & $13.1$ & 
        $-1.8$ & $3.2$ & 
        %$13.75$ & $15.56$ & 
        $9.3$ & $21.1$ & 
        $33.0$ & $0.2$ & 
        $\mathbf{34.1}$ & $0.1$ &
        $-1.2$ & $3.0$ \\
        & \texttt{mount-car} & 
        $81.2$ & $0.3$ & 
        %$84.42$ & $4.88$ & 
        $\mathbf{85.1}$ & $1.8$ & 
        %$86.23$ & $1.86$ & 
        $11.4$ & $34.1$ & 
        $9.6$ & $35.3$ & 
        $-21.3$ & $2.9$ &
        $-30.0$ & $35.5$ \\
        & \texttt{road} & 
        $\mathbf{22.7}$ & $0.0$ & 
        %$22.74$ & $0.001$ & 
        $\mathbf{22.7}$ & $0.0$ & 
        %$22.74$ & $0.01$ & 
        $9.7$ & $16.4$ & 
        $\mathbf{22.7}$ & $0.0$ & 
        $\mathbf{22.7}$ & $0.05$ &
        $\mathbf{22.7}$ & $0.0$  \\
        & \texttt{road2d} & 
        $\mathbf{24.0}$ & $0.2$ & 
        %$24.18$ & $0.08$ & 
        $\mathbf{24.0}$ & $0.2$ & 
        %$24.08$ & $0.19$ & 
        $11.2$ & $16.5$ & 
        $\mathbf{24.0}$ & $0.0$ & 
        $\mathbf{24.0}$ & $0.1$ &
        $\mathbf{24.0}$ & $0.1$  \\
        \hline
        \multirow{4}{*}{\rotatebox{0}{{DI}}}                      
        & \texttt{dynamic-obs} & 
        $\mathbf{13.2}$ & $0.0$ & 
        %$13.12$ & $0.11$ & 
        $-1.3$ & $1.9$ & 
        %$12.56$ & $0.81$ & 
        \;- & \;- & 
        $-21.4$ & $21.1$ & 
        $-4.2$ & $24.9$ &
        $-5.0$ & $0.3$ \\
        & \texttt{single-gate} & 
        $\mathbf{11.6}$ & $0.0$ & 
        %$11.64$ & $0.01$ & 
        $\mathbf{11.6}$ & $0.0$ & 
        %$11.64$ & $0.02$ & 
        \;- & \;- & 
        $-19.6$ & $17.0$ &
        $-2.0$ & $1.1$ &
        $-2.1$ & $0.2$  \\
        & \texttt{double-gates} & 
        $\mathbf{12.7}$ & $1.0$ & 
        %$12.39$ & $1.48$ & 
        $11.5$ & $1.1$ & 
        %$11.16$ & $1.79$ & 
        \;- & \;- & 
        $-6.7$ & $5.4$ &
        $-3.9$ & $11.1$ &
        $-3.6$ & $1.0$  \\
        & \texttt{double-gates+} & 
        $\mathbf{13.0}$ & $0.6$ & 
        %$3.84$ & $3.91$ & 
        $-0.9$ & $0.1$ & 
        %$8.46$ & $3.26$ & 
        \;- & \;- & 
        $-17.4$ & $12.8$ &
        $-2.8$ & $0.4$ &
        $-4.1$ & $1.1$ \\
        \hline
        \multirow{4}{*}{\rotatebox{0}{{DD}}}                        
        & \texttt{dynamic-obst} & 
        $\textbf{7.4}$ & $3.7$ & 
        %c & d & 
        $6.3$ & $2.1$ & 
        %g & h & 
        \;- & \;- & 
        $-4.5$ & $0.5$ &
        $-3.6$ & $0.8$ &
        $-5.3$ & $0.5$ \\
        & \texttt{single-gate} & 
        $\mathbf{11.5}$ & $0.1$ & 
        %$11.52$ & $0.04$ & 
        $11.4$ & $0.1$ & 
        %$11.58$ & $0.02$ & 
        \;- & \;- & 
        $-2.5$ & $0.3$ &
        $-2.4$ & $0.2$ &
        $-3.1$ & $0.5$  \\
        & \texttt{double-gates} & 
        $\mathbf{13.1}$ & $0.5$ & 
        %$13.3$ & $0.07$ & 
        $10.9$ & $1.8$ & 
        %$12.64$ & $0.62$ & 
        \;- & \;- & 
        $-2.4$ & $0.6$ &
        $-1.9$ & $0.9$ &
        $-3.4$ & $0.5$  \\
        & \texttt{double-gates+} & 
        $\mathbf{13.0}$ & $0.6$ & 
        %$11.54$ & $1.73$ & 
        $8.5$ & $2.3$ & 
        %$10.68$ & $1.58$ & 
        \;- & \;- & 
        $-2.5$ & $0.3$ &
        $-20.7$ & $22.8$ &
        $-3.6$ & $0.3$  \\
      %  \hline
      %  & \texttt{average} & 
      %  a & b & 
      %  A & & 
      %  c & Y & 
      %  d & X & 
      %  e & Z & 
      %  f & Y & 
      %  g & X \\
        \hline
    \end{tabular}
\end{table}


==> files/safety_table_rebuttal.tex <==
\newlength{\colwidthXX}
\setlength{\colwidthXX}{5mm} % You can adjust the value as needed

\begin{table}[h]
    \centering
    \scriptsize
    \caption*{Table 1: Updated Safety Results}
    \label{tab:safety}
    \begin{tabular}{|cl|rr|rr|rr|rr|rr|rr|}
        \hline
        \multicolumn{2}{|c|}{\multirow{3}{*}{\bf Benchmark}} & 
        \multicolumn{6}{c|}{\textbf{\# Shield Invocations / Episode}} & 
        \multicolumn{6}{c|}{\textbf{\# Safety Violations / Episode}} \\ \cline{3-14} 
        &           & 
        \multicolumn{2}{|c|}{\tool} & 
        %\multicolumn{2}{|c|}{\texttt{DMPS-H1}}  & 
        \multicolumn{2}{|c|}{\texttt{MPS}} & 
        %\multicolumn{2}{|c|}{\texttt{DMPS-G}}  & 
        \multicolumn{2}{|c|}{\texttt{REVEL}}  & 
        \multicolumn{2}{|c|}{\texttt{CPO}}  &
        \multicolumn{2}{|c|}{\texttt{PPO-lag}}  &
        \multicolumn{2}{|c|}{\texttt{TD3}} \\
        &           & 
        mean & sd & 
        mean & sd &  
        %mean & sd & 
        mean & sd &  
        mean & sd &  
        mean & sd &  
        mean & sd \\
        \hline
        \multirow{5}{*}{\rotatebox{0}{ST}} 
        & \texttt{obstacle} & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & Z & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & X & 
        $4.0$ & $8.0$ & 
        $\mathbf{0.0}$ & $0.0$ & 
        $\mathbf{0.0}$ & $0.0$ &
        $\mathbf{0.0}$ & $0.0$ \\
        & \texttt{obstacle2} & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$2.8$ & 5.6 & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$13.71$ & 27.4 & 
        $33.8$ & $30.3$ & 
        $0.9$ & $0.2$ & 
        $6.42$ & $0.19$ &
        $\mathbf{0.0}$ & $0.0$ \\
        & \texttt{mount-car} & 
        $\mathbf{0.0}$ & $0.0$ & 
        %b & Z & 
        $\mathbf{0.0}$ & $0.0$ & 
        %d & X & 
        $4.0$ & $4.0$ & 
        $2.0$ & $2.1$ &
        $22.2$ & $28.9$ &
        $\mathbf{0.0}$ & $0.0$ \\
        & \texttt{road} & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & Z & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & X & 
        $0.8$ & $0.74$ & 
        $\mathbf{0.0}$ & $0.0$ & 
        $\mathbf{0.0}$ & $0.0$ &
        $\mathbf{0.0}$ & $0.0$ \\
        & \texttt{road2d} & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & Z & 
        $\mathbf{0.0}$ & $0.0$ & 
        %$0.0$ & X & 
        $\mathbf{0.0}$ & $0.0$ & 
        $\mathbf{0.0}$ & $0.0$ &
        $\mathbf{0.0}$ & $0.0$ &
        $\mathbf{0.0}$ & $0.0$ \\
        \hline
        \multirow{4}{*}{\rotatebox{0}{{DI}}}                      
        & \texttt{dynamic-obst} & 
        $\mathbf{9.3}$ & $1.8$ & 
        %b & Z & 
        $144.1$ & $26.2$ & 
        %d & X & 
        \;- & \;- & 
        $1.7$ & $0.8$ &
        $3.6$ & $3.9$ &
        $\mathbf{0.8}$ & $1.2$ \\
        & \texttt{single-gate} & 
        $\mathbf{0.1}$ & $0.0$ & 
        %$0.15$ & 0.1 & 
        $0.2$ & $0.1$ & 
        %$0.12$ & 0.1 & 
        \;- & \;- & 
        $2.0$ & $1.2$ &
        $10.0$ & $5.5$ &
        $\mathbf{0.0}$ & $0.0$ \\
        & \texttt{double-gates} & 
        $\mathbf{4.5}$ & $1.2$ & 
        %$6.38$ & 1.5 & 
        $28.3$ & $6.9$ & 
        %$19.84$ & 4.5 & 
        \;- & \;- & 
        $2.1$ & $1.7$ & 
        $11.8$ & $6.3$ &
        $\mathbf{0.3}$ & $0.5$ \\
        & \texttt{double-gates+} & 
        $\mathbf{24.2}$ & $6.4$ & 
        %$124.38$ & 16.3 & 
        $239.8$ & $16.3$ & 
        %$89.47$ & 36 & 
        \;- & \;- & 
        $2.9$ & $1.0$ & 
        $6.5$ & $4.5$ &
        $\mathbf{0.0}$ & $0.0$ \\
        \hline
        \multirow{4}{*}{\rotatebox{0}{{DD}}}                        
        & \texttt{dynamic-obst} & 
        $\textbf{105.2}$ & $39.9$ & 
        %b & Z & 
        $144.9$ & $39.9$ & 
        %d & X & 
        \;- & \;- & 
        $1.7$ & $1.9$ & 
        $2.9$ & $2.2$ &
        $\mathbf{0.8}$ & $0.16$ \\
        & \texttt{single-gate} & 
        $\mathbf{3.1}$ & $1.6$ & 
        %$4.52$ & 4.5 & 
        $7.4$ & $6.9$ & 
        %$3.44$ & 2.4 & 
        \;- & \;- & 
        $5.2$ & $3.5$ & 
        $6.7$ & $7.2$ &
        $\mathbf{0.1}$ & $0.2$ \\
        & \texttt{double-gates} & 
        $\mathbf{5.5}$ & $1.9$ & 
        %$7.15$ & 2.5 & 
        $52.5$ & $17.6$ & 
        %$34.06$ & 12.9 & 
        \;- & \;- & 
        $3.9$ & $1.7$ & 
        $7.9$ & $9.2$ &
        $\mathbf{3.0}$ & $5.5$ \\
        & \texttt{double-gates+} & 
        $\mathbf{18.4}$ & $13.0$ & 
        %$34.68$ & 29.5 & 
        $106.2$ & $18.5$ & 
        %$89.4$ & 32.7 & 
        \;- & \;- & 
        $12.1$ & $2.9$ &
        $6.9$ & $6.1$ &
        $\mathbf{0.2}$ & $0.4$ \\
        \hline
   %     & \texttt{average} & 
   %     a & b & 
   %     %A & & 
   %     c & Y & 
   %     %d & X & 
   %     \;- & \;- & 
   %     f & Y & 
   %     g & X \\
   %     \hline
    \end{tabular}
\end{table}


==> performance_plots.tex <==
\setlength{\figheight}{28mm} % Adjust the value as needed
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/Gate_DoubleIntegrator.png}}
        \caption*{\texttt{dynamic-obs\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/Gate_DoubleIntegrator.png}}
        \caption*{\texttt{single-gate\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/DoubleGate_DoubleIntegrator.png}}
        \caption*{\texttt{double-gate\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_DoubleIntegrator.png}}
        \caption*{\texttt{double-gate+\,(DI)}}
        \label{}
    \end{subfigure}
    %
%
%
%
        \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/Gate_Steering.png}}
        \caption*{\texttt{dynamic-obs\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/Gate_Steering.png}}
         \caption*{\texttt{single-gate\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/DoubleGate_Steering.png}}
         \caption*{\texttt{double-gate\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{rew_plots/ThickDoubleGate_Steering.png}}
         \caption*{\texttt{double-gate+\,(DD)}}
        \label{}
    \end{subfigure}
    \caption{Performance Results on Dynamic Benchmarks \red{plots show outdated results. to be updated. plots for dynamic-obs are placeholders} }
    \label{fig:performance_plots}
\end{figure}


==> shield_plots.tex <==
\setlength{\figheight}{28mm} % Adjust the value as needed
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/Gate_DoubleIntegrator.png}}
        \caption*{\texttt{dynamic-obs\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/Gate_DoubleIntegrator.png}}
        \caption*{\texttt{single-gate\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/DoubleGate_DoubleIntegrator.png}}
        \caption*{\texttt{double-gate\,(DI)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_DoubleIntegrator.png}}
        \caption*{\texttt{double-gate+\,(DI)}}
        \label{}
    \end{subfigure}
    %
%
%
%
        \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/Gate_Steering.png}}
        \caption*{\texttt{dynamic-obs\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/Gate_Steering.png}}
         \caption*{\texttt{single-gate\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/DoubleGate_Steering.png}}
         \caption*{\texttt{double-gate\,(DD)}}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \makebox[0pt]{\includegraphics[height=\figheight, keepaspectratio]{shield_plots/ThickDoubleGate_Steering.png}}
         \caption*{\texttt{double-gate+\,(DD)}}
        \label{}
    \end{subfigure}
    \caption{Shield Trigger Rates on Dynamic Benchmarks \red{plots show outdated results. to be updated}}
    \label{fig:shield_plots}
\end{figure}

